New Perspectives on the Evaluation of Link Prediction Algorithms for Dynamic Graphs

There is a fast-growing body of research on predicting future links in dynamic networks, with many new algorithms. Some benchmark data exists, and performance evaluations commonly rely on comparing the scores of observed network events (positives) with those of randomly generated ones (negatives). These evaluation measures depend on both the predictive ability of the model and, crucially, the type of negative samples used. Besides, as generally the case with temporal data, prediction quality may vary over time. This creates a complex evaluation space. In this work, we catalog the possibilities for negative sampling and introduce novel visualization methods that can yield insight into prediction performance and the dynamics of temporal networks. We leverage these visualization tools to investigate the effect of negative sampling on the predictive performance, at the node and edge level. We validate empirically, on datasets extracted from recent benchmarks that the error is typically not evenly distributed across different data segments. Finally, we argue that such visualization tools can serve as powerful guides to evaluate dynamic link prediction methods at different levels.

==> dataset_stats.tex <==
% \usepackage{booktabs}

% \begin{table}
%     \caption{Sample table title}
%     \label{sample-table}
%     \centering
%     \begin{tabular}{lll}
%       \toprule
%       \multicolumn{2}{c}{Part}                   \\
%       \cmidrule(r){1-2}
%       Name     & Description     & Size ($\mu$m) \\
%       \midrule
%       Dendrite & Input terminal  & $\sim$100     \\
%       Axon     & Output terminal & $\sim$10      \\
%       Soma     & Cell body       & up to $10^6$  \\
%       \bottomrule
%     \end{tabular}
%   \end{table}


% \begin{table}
%     \centering
%     \begin{tabular}{|l|lrrrrr|} 
%     \toprule
%     Dataset   & Type       & $N_nodes$ & $\bar{T}_{min}^{(node)}$ & $\bar{T}_{min}^{(sender)}$ & $\bar{T}_{min}^{(receiver)}$ & Asymmetry  \\ 
%     \midrule
%     lastfm    & Bipartite  & 1981      & 0.27                     & 0.42                       & 0.13                         & -0.29      \\
%     wikipedia & Bipartite  & 9228      & 0.38                     & 0.40                       & 0.18                         & -0.23      \\
%     enron     & Directed   & 185       & 0.41                     & 0.50                       & 0.42                         & -0.08      \\
%     reddit    & Bipartite  & 10985     & 0.09                     & 0.10                       & 0.03                         & -0.07      \\
%     SocialEvo & Undirected & 75        & 0.03                     & 0.06                       & 0.04                         & -0.02      \\
%     Flights   & Directed   & 13170     & 0.11                     & 0.15                       & 0.13                         & -0.02      \\
%     UNtrade   & Directed   & 256       & 0.05                     & 0.05                       & 0.05                         & -0.01      \\
%     USLegis   & Undirected & 226       & 0.32                     & 0.32                       & 0.32                         & 0.00       \\
%     UNvote    & Undirected & 202       & 0.27                     & 0.27                       & 0.27                         & -0.00      \\
%     uci       & Directed   & 1900      & 0.18                     & 0.18                       & 0.19                         & 0.01       \\
%     Contacts  & Undirected & 693       & 0.08                     & 0.08                       & 0.09                         & 0.01       \\
%     mooc      & Bipartite  & 7145      & 0.28                     & 0.28                       & 0.44                         & 0.16       \\
%     CanParl   & Undirected & 735       & 0.31                     & 0.31                       & 0.48                         & 0.17       \\
%     \bottomrule
%     \end{tabular}
% \end{table}
% \begin{table}
%     \caption{Arrival times for each dataset}
%     \label{tab:arrival_times}
%     \begin{tabular}{llrrrrrrrr}
%     \toprule
%      &  & avg_nat & avg_sat & avg_rat & asymmetry & n_nodes & n_interactions & n_oriented_edges & n_undirected_edges \\
%     Type & dataset &  &  &  &  &  &  &  &  \\
%     \midrule
%     \multirow[t]{4}{*}{Bipartite} & lastfm & 0.27 & 0.42 & 0.13 & -0.29 & 1981 & 1293103 & 154993 & 154993 \\
%      & mooc & 0.28 & 0.28 & 0.44 & 0.16 & 7145 & 411749 & 178443 & 178443 \\
%      & reddit & 0.09 & 0.10 & 0.03 & -0.07 & 10985 & 672447 & 78516 & 78516 \\
%      & wikipedia & 0.38 & 0.40 & 0.18 & -0.23 & 9228 & 157474 & 18257 & 18257 \\
%     \midrule
%     \multirow[t]{4}{*}{Directed} & Flights & 0.11 & 0.15 & 0.13 & -0.02 & 13170 & 1927145 & 395072 & 301770 \\
%      & UNtrade & 0.05 & 0.05 & 0.05 & -0.01 & 256 & 507497 & 36182 & 20701 \\
%      & enron & 0.41 & 0.50 & 0.42 & -0.08 & 185 & 125235 & 3125 & 2215 \\
%      & uci & 0.18 & 0.18 & 0.19 & 0.01 & 1900 & 59835 & 20296 & 13838 \\
%     \midrule
%     \multirow[t]{5}{*}{Undirected} & CanParl & 0.31 & 0.31 & 0.48 & 0.17 & 735 & 74478 & 51331 & 45697 \\
%      & Contacts & 0.08 & 0.08 & 0.09 & 0.01 & 693 & 2426279 & 79530 & 79530 \\
%      & SocialEvo & 0.03 & 0.06 & 0.04 & -0.02 & 75 & 2099519 & 4486 & 2506 \\
%      & UNvote & 0.27 & 0.27 & 0.27 & -0.00 & 202 & 1035742 & 31516 & 19722 \\
%      & USLegis & 0.32 & 0.32 & 0.32 & 0.00 & 226 & 60396 & 26423 & 16667 \\
%     \midrule
%     \bottomrule
%     \end{tabular}
%     \end{table}
% "$\bar{T}_{min}^{(node)}$",
% "$\bar{T}_{min}^{(sender)}$ ",
% "$\bar{T}_{min}^{(receiver)}$",
% "Asymmetry",
% "$N_{nodes}$",
% "$N_{interactions}$",
% "$N_{oriented}$",
% "$N_{undirected}$",


\resizebox{\columnwidth}{!}{%
    \begin{tabular}{{llrrrrrrr}}
        \toprule
                                       &           & Nodes & Interactions & \makecell{Directed \\ Edges} & \makecell{Undirected\\ Edges}   & $\bar{T}_{min}^{(sender)}$ & $\bar{T}_{min}^{(receiver)}$ & Asymmetry \\
        Type                           & Dataset    &       &              &                &                    &                            &                              &           \\
        \midrule
        \multirow[t]{4}{*}{Bipartite}  & lastfm  & 1981  & 1293103      & 154993         & 154993             & 0.42                       & 0.13                         & -0.29     \\
                                       & mooc      & 7145  & 411749       & 178443         & 178443             & 0.28                       & 0.44                         & 0.16      \\
                                       & reddit    & 10985 & 672447       & 78516          & 78516              & 0.10                       & 0.03                         & -0.07     \\
                                       & wikipedia & 9228  & 157474       & 18257          & 18257              & 0.40                       & 0.18                         & -0.23     \\
        \midrule
        \multirow[t]{4}{*}{Directed}   & Flights   & 13170 & 1927145      & 395072         & 301770             & 0.15                       & 0.13                         & -0.02     \\
                                       & UNtrade   & 256   & 507497       & 36182          & 20701              & 0.05                       & 0.05                         & -0.01     \\
                                       & enron     & 185   & 125235       & 3125           & 2215               & 0.50                       & 0.42                         & -0.08     \\
                                       & uci       & 1900  & 59835        & 20296          & 13838              & 0.18                       & 0.19                         & 0.01      \\
        \midrule
        \multirow[t]{5}{*}{Undirected} & CanParl   & 735   & 74478        & 51331          & 45697              & 0.31                       & 0.48                         & 0.17      \\
                                       & Contacts  & 693   & 2426279      & 79530          & 79530              & 0.08                       & 0.09                         & 0.01      \\
                                       & SocialEvo & 75    & 2099519      & 4486           & 2506               & 0.06                       & 0.04                         & -0.02     \\
                                       & UNvote    & 202   & 1035742      & 31516          & 19722              & 0.27                       & 0.27                         & -0.00     \\
                                       & USLegis   & 226   & 60396        & 26423          & 16667              & 0.32                       & 0.32                         & 0.00      \\

        \bottomrule
    \end{tabular}
}

% & $\bar{T}_{min}^{(node)}$
% &                         
% & 0.27                    
% & 0.28                    
% & 0.09                    
% & 0.38                    
% & 0.11                    
% & 0.05                    
% & 0.41                    
% & 0.18                    
% & 0.31                    
% & 0.08                    
% & 0.03                    
% & 0.27                    
% & 0.32                    
